Joint Planning of Charging Stations and Power Systems for Heavy-Duty Drayage Trucks

As global concerns about climate change intensify, the transition towards zero-emission freight is becoming increasingly vital. Drayage is an important segment of the freight system, typically involving the transport of goods from seaports or intermodal terminals to nearby warehouses. This sector significantly contributes to not only greenhouse gas emissions, but also pollution in densely populated areas. This study presents a holistic optimization model designed for an efficient transition to zero-emission drayage, offering cost-effective strategies for the coordinated investment planning for power systems, charging infrastructure, and electric drayage trucks. The model is validated in the Greater Los Angeles area, where regulatory goals are among the most ambitious. Furthermore, the model's design allows for easy adaptation to other regions. By focusing on drayage trucks, this study also paves the way for future research into other freight categories, establishing a foundation for a more extensive exploration in this field.

==> history/4-model-with-exact-charger-levels.tex <==
\section{Model Formulation}
\label{sec:model}

\subsection{Problem Description}
\label{sec:problem-description}

\begin{table}[!h]
\caption{Summary of notations for sets, parameters, and decision variables.}
\begin{center}
\begin{threeparttable}
\begin{tabular}{ l l }
    \toprule
     &  \textbf{Sets} \\
    $I$ & Set of trucks.\\
    $J$ & Set of candidate charging stations.\\
    $K$ & Set of electric substations.\\
    $M$ & Set of candidate charger types.\\
    $T$ & Set of time steps of the study time horizon.\\
    $J_{it}$ & Subset of $J$ that truck $i$ has access to at time step $t$.\\
    $J_k$ & Subset of $J$ that can be connected with electric substation $k$.\\
    $K_j$ & Subset of $K$ that can be connected with charging station $j$.\\
    $T^{prk}_{i}$ & Subset of $T$ at which truck $i$ is parked.\\
    % $T^{depot}_{i}$ & Subset of $T$ at which truck $i$ is parking in its depot.\\
     &  \textbf{Parameters} \\
    $u_{i}$ & Daily carbon emission of truck $i$ if it uses diesel as the fuel.\\
    $g_t$ & Electricity carbon intensity of the grid at time $t$.\\
    $e^{bse}$ & Base battery capacity of an electric truck before upgrading.\\
    $SoC^{min}/SoC^{max}$ & Minimal/maximal allowed state-of-charge of an electric truck.\\
    $x^{max,m}$ & Maximal charging power of a type $m$ charger.\\
    $s_{it}$ & Power consumption rate of truck $i$ at time $t$.\\
    $\eta$ & Energy efficiency of electric trucks.\\
    $\kappa$ & Cycle efficiency of charging batteries.\\
    $\beta_{ijt}$ & $\beta_{ijt} = 1$ indicates truck $i$ has access to candidate charging station $j$ at time $t$. Otherwise, $\beta_{ijt} = 0$.\\
    $P^{sbs}_{k}$ & Remaining hosting power capacity of electric substation $k$.\\
    $d_{jk}$ & Distance between charging station $j$ and electric substation $k$.\\
    $c^{lne}$ & Cost of distribution line between a charging station and an electric substation (per mile basis).\\
    $c^{chg,m}$ & Cost of one type $m$ charger.\\
    $c^{pwr}$ & Cost of providing one kW of power capacity at a charging station.\\
    $c^{fix}$ & Cost of charging station make-ready, including licensing, construction, etc.\\
    $c^{trk}$ & Cost of one electric truck.\\
    $c^{ele}_t$ & Cost of 1kWh electricity at time $t$.\\
    $c^{btr}$ & Cost of adding 1kWh of extra battery capacity.\\
    $c^{deg}$ & Cost of battery degradation by charging 1kWh of electricity.\\
    $B$ & Budget.\\
    \\
    & \textbf{Decision Variables$^*$} \\
    $U$ & (C) Daily GHG emission of the truck sector.\\
    $z_{i}$ & (B) $z_{i} = 1$ indicates truck $i$ is electrified. Otherwise, $z_{i} = 0$.\\
    $e^{cap}_{i}$ & (C) Required battery capacity of truck $i$.\\
    $x_{it}$ & (C) Charging power on truck $i$ at time $t$.\\
    $P^{chs}_{j}$ & (C) Power capacity of charging station $j$.\\
    $p_{jt}$ & (C) Power demand of trucks in charging station $j$ at time $t$.\\
    $N^{m}_{j}$ & (I) Number of type $m$ chargers installed at charging station $j$.\\
    $n^{m}_{kt}$ & (I) Number of type $m$ chargers in-use at charging station $j$ at time $t$.\\
    $x^{m}_{ijt}$ & (B) $x^{m}_{ijt} = 1$ indicates the need of one type $m$ charger for truck $i$ at location $j$ at time $t$.\\
    $\hat N_{j}$ & (B) $\hat N_{j} = 1$ indicates the candidate charging station $j$ is deployed. Otherwise, $\hat N_{j} = 0$.\\
    $\gamma_{jk}$ & (B) $\gamma_{jk} = 1$ charging station $j$ is connected to electric substation $k$. Otherwise, $\gamma_{jk} = 0$.\\
    \bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
\item[*] (C) Continuous variable; (B) Binary variable; (I) Integer variable.
\end{tablenotes}
\end{threeparttable}
\end{center}
\label{tab:params}
\end{table}

\subsection{Objective Function}

The objective function is the minimization of the total GHG emissions from the electric and diesel trucks: 

\begin{equation}
    \underset{}{\text{min}} \ U^{t},
\label{eq:objective}
\end{equation}

\begin{equation}
    U^{t} = \sum_{i \in I}(1-z_i)\cdot u^{t}_i + \sum_{i \in I}\sum_{t \in T}g_t \cdot x_{it} \cdot \Delta t,
\label{eq:Ub}
\end{equation}

\subsection{Constraints}

\subsubsection{Energy}

\eqref{eq:e-cont} ensures the continuous change of battery energy levels. \eqref{eq:e-range} ensures the range of battery energy levels. \eqref{eq:x-range} ensures the range of charging powers. \eqref{eq:x-zero} ensures when the truck is not parking or when it does not have access to a candidate charging station, the charging power is zero.

\begin{equation}
    e_{it^{\prime}} = e_{it} + x_{it} \cdot \Delta t - z_i \cdot s_{it} , \quad \forall i \in I, \forall t \in T, t^{\prime} = Next(t)
\label{eq:e-cont}
\end{equation}

\begin{equation}
e^{min} \leq e_{it} \leq e^{max}, \quad \forall i \in I, \forall t \in T,
\label{eq:e-range}
\end{equation}

\begin{equation}
    0 \leq x_{it} \leq z_i \cdot x^{max}, \quad \forall i \in I, \forall t \in T,
\label{eq:x-range}
\end{equation}

\begin{equation}
    x_{it} = 0, \quad \forall i \in I, \forall t \notin T^{prk}_i \text{ or } \sum_{j\in J_{it}} \beta_{ijt} = 0,
\label{eq:x-zero}
\end{equation}

\begin{equation}
    z_i \in \{0, 1\}, \quad \forall i \in I,
\label{eq:z-def}
\end{equation}

\subsubsection{Power Capacity Limit of Charging Stations}

\eqref{eq:Pjt1} and \eqref{eq:Pjt2} ensure that the total charging power of a charging station is less than the power capacity of the charging station at any time.

\begin{equation}
    P_{jt} \leq P^{chs}_{j} , \quad \forall j \in J, \forall t \in T,
\label{eq:Pjt1}
\end{equation}

\begin{equation}
    P_{jt} = \sum_{i \in I_{jt}} \beta_{ijt} x_{it}, \quad \forall j \in J, \forall t \in T,
\label{eq:Pjt2}
\end{equation}

\subsubsection{Number of Chargers}
Suppose a charging station can choose from a set of $M$ types of chargers, featuring different charging powers. For the type $m$ charger, its maximum power is $p^m$. For example, suppose the set $M$ consists of two types of chargers with 350kW and 500kW charging power respectively, then $p^1 = $350kW and $p^2 = $500kW. \eqref{eq:nmjt1} and \eqref{eq:nmjt2} ensure that the number of type $m$ chargers in use at a charging station $j$ ($n^{m}_{jt}$) is less than the installed type $m$ chargers ($N^{m}_{j}$) at any time. $\hat x^{m}_{ijt}$ indicates the use of type $m$ chargers by truck $i$ at time $t$ in charging station $j$ as defined in \eqref{eq:hatx}. When $m=1$, we set $p^0=0kW$. 

\begin{equation}
    n^{m}_{jt} \leq N^{m}_{j}, \quad \forall j \in J, \forall t \in T, \forall m \in M
\label{eq:nmjt1}
\end{equation}

\begin{equation}
    n^{m}_{jt} = \sum_{i \in I_{jt}} \hat x^{m}_{ijt}, \quad \forall j \in J, \forall t \in T,
\label{eq:nmjt2}
\end{equation}

\begin{equation}
\hat x^{m}_{ijt} =
\begin{cases}
    1, & \text{if $p^{m-1} < \beta_{ijt}x_{it} \leq p^{m}$}\\
    0, & \text{otherwise},
\end{cases}, \forall (i, j, t, m) \in (I, J, T, M)
\label{eq:hatx}
\end{equation}

Referring to \ref{ap:linear} about how \eqref{eq:hatx} is linearized.

\subsubsection{Investment Decision on Candidate Charging Stations}
If the number of chargers in a candidate charging station $j$ is greater than 0, this candidate location will be selected for actual deployment as indicated by binary variable $\hat N_{j}$.

\begin{equation}
\hat N_{j} =
\begin{cases}
    1, & \text{if $\sum_{m \in M}N^{m}_{j} > 0$}\\
    0, & \text{otherwise}
\end{cases}, \forall j \in J
\label{eq:hat-N}
\end{equation}

\subsubsection{Spatial Constraints of Trucks}

\eqref{eq:hatx-spt} ensures that a truck $i$ can only utilize one charging station and one charger at a time $t$.

\begin{equation}
\sum_{j \in J_{it}}\sum_{m \in M} \hat x^{m}_{ijt} \leq 1, \quad \forall i \in I, \forall t \in T,
\label{eq:hatx-spt}
\end{equation}

When a truck is parked at $t$ and getting charged at a charging station $j_0$, then for practical considerations, it will be staying at this charging station throughout the charging session. In other words, a continuous charging session should be performed in only one location. \eqref{eq:loc} ensures this logic is satisfied. The first term of the left-hand side (LHS) of \eqref{eq:loc} indicates a charging session happens at location $j_0$ during time step $t$, while the second term indicates a charging session happens at locations other than $j_0$ during the subsequent time step $t^{\prime}$. Note that switching charger types is allowed within the same charging station.

% \begin{equation}
% \sum_{m \in M} \hat x^{m}_{ij_0t} + \sum_{j \in J_{it^{\prime}}\setminus{j_0}}\sum_{m \in M} \hat x^{m}_{ijt^{\prime}} \leq 1, \quad \forall i \in I, \forall j_0 \in J_{it} \cap J_{it^{\prime}}, \forall t \in T,
% \label{eq:loc}
% \end{equation}

% \begin{equation}
% \sum_{m \in M} \hat x^{m}_{ij_0t} + \sum_{j \in J_{it^{\prime}}\setminus{j_0}}\sum_{m \in M} \hat x^{m}_{ijt^{\prime}} \leq 1, \quad \forall (i, j_0, t, t^{\prime}) \in (I, J_{it} \cap J_{it^{\prime}}, T^{prk}, T^{prk})
% \label{eq:loc}
% \end{equation}

\begin{equation}
\sum_{m \in M} \hat x^{m}_{ijt} + \sum_{j^{\prime} \in J_{it^{\prime}}\setminus{j}}\sum_{m \in M} \hat x^{m}_{ij^{\prime}t^{\prime}} \leq 1, \quad \forall (i, j, t) \in (I, J_{it} \cap J_{it^{\prime}}, T^{prk}), t^{\prime} = Next(t)
\label{eq:loc}
\end{equation}

\subsubsection{Power Capacity Limit of an Electric Substation}

To source electricity from the grid, a charging station needs to be connected to an electric substation. Otherwise, the charging station will not have any power capacity, as ensured in \eqref{eq:Pchs}, where $\gamma_{j,k}$ indicates the existence of a connection between charging station $j$ and electric substation $k$. Also, a charging station can only connect to one electric substation for practical considerations, as ensured by \eqref{eq:gamma}.

\begin{equation}
    P^{chs}_{j} \leq \sum_{k \in K_j} \gamma_{jk} \cdot G, \quad \forall j \in J,
\label{eq:Pchs}
\end{equation}

\begin{equation}
    \sum_{k \in K_j} \gamma_{jk} \leq 1, \quad \forall j \in J,
\label{eq:gamma}
\end{equation}

On the other hand, an electric substation has its own limit of remaining hosting power capacity $P^{sbs}_{k}$, and the cumulative power capacity required by charging stations it connects with shall not exceed this limit, as ensured by \eqref{eq:Psbs}.

\begin{equation}
    \sum_{j \in J_k} \gamma_{jk} P^{chs}_{j} \leq P^{sbs}_{k}, \quad \forall k \in K,
\label{eq:Psbs}
\end{equation}

\subsubsection{Budget}

The overall project is constrained by a given budget $B$, while the costs include:

\begin{itemize}
    \item Cost of connection between charging stations and electric substations depends on the unit cost of power lines $c^{lne}$ and the distance between two locations $d_{jk}$.
    \item Cost of charging station includes fixed civil construction and licensing cost ($c^{fix} \cdot \hat N_{j}$), power equipment cost ($c^{pwr} \cdot P^{chs}_{j}$), and charger cost ($\sum_{m \in M}c^{chg,m} \cdot N^{m}_j$).
    \item Cost of purchasing electric trucks ($c^{trk} \cdot z_i$) and any battery upgrade needed ($c^{btr} \cdot \left(e^{cap}_{i}-e^{bse}\right)$).
    \item Cost of electricity subject to the daily variation of electricity price $c^{ele}_t$.
\end{itemize}

\begin{flalign}
    &\qquad\underbrace{\sum_{j \in J}\sum_{k \in K_j}c^{lne} \cdot \gamma_{jk} \cdot d_{jk}}_{\text{Cost of connection to substation}}
    + \ \underbrace{\sum_{j \in J} (c^{fix} \cdot \hat N_{j} + c^{pwr} \cdot P^{chs}_{j} + \sum_{m \in M}c^{chg,m} \cdot N^{m}_j)}_{\text{Cost of charging station}} 
    +\label{eq:budget}  & \\
    &\qquad\qquad\qquad\qquad\quad \underbrace{\sum_{i \in I}\left[c^{trk} \cdot z_i + c^{btr} \cdot \left(e^{cap}_{i}-e^{bse}\cdot z_i\right)\right]}_{\text{Cost of electric truck and battery upgrades}}
    +
    \underbrace{D\sum_{t \in T} \sum_{i \in I}c^{ele}_t \cdot x_{it}\Delta t}_{\text{Cost of electricity}}\leq B. \nonumber
\end{flalign}


\subsection{Summary of the Model}

As a summary of the model formulation in this section, the model is solved under objective function \eqref{eq:objective} and subject to constraints \eqref{eq:Ub} - \eqref{eq:EV-cost}. Specifically, \eqref{eq:hat-x}, \eqref{eq:hat-y} and \eqref{eq:hat-N} will be \textcolor{blue}{linearized} using standard techniques \textcolor{blue}{(see Appendix \ref{ap:linear})} such that the optimization problem is transformed to a mixed-integer linear program (MILP), which can be handled by commercial solvers. 




% Both EB and EV are in public budget
% \begin{equation}
%     \sum_{k \in K} (c^b N^{b}_k + c^v N^{v}_k  + c^f \hat N_{k} + c^p P_{k}) + \sum_{i \in I}c^{eb} z_i + \textcolor{blue}{D\sum_{t \in T} \left [c^{e}_t \left (\sum_{i \in I}x_{it} + \sum_{j \in J}y_{jt} \right)\Delta t \right ]} \leq B,
% \label{eq:budget}
% \end{equation}

% Not net-metering
% \begin{equation}
%     \sum_{k \in K} (c^b N^{b}_k + c^v N^{v}_k  + c^f \hat N_{k} + c^p P_{k}) + \sum_{i \in I}c^{eb} z_i + \textcolor{blue}{D\sum_{t \in T} \left [c^{e,buy}_t max(P_{kt}, 0) + c^{e,sell}_t min(P_{kt}, 0)\Delta t \right ]} \leq B,
% \label{eq:budget}
% \end{equation}

% Subsidy degradation
% \begin{equation}
%     \sum_{k \in K} (c^b N^{b}_k + c^v N^{v}_k  + c^f \hat N_{k} + c^p P_{k}) + \sum_{i \in I}c^{eb} z_i + \textcolor{blue}{D\sum_{t \in T} \left [\sum_{i \in I}c^{e}_t x_{it} \Delta t + \sum_{j \in J}c^{deg} min(y_{jt},0)\right ]} +  \leq B,
% \label{eq:budget}
% \end{equation}

% \begin{equation}
%      \textcolor{blue}{D\sum_{t \in T} \sum_{j \in J}c^{e}_t y_{jt}\Delta t \leq C^{EV}_{min}},
% \label{eq:EV-cost}
% \end{equation}

==> history/Parameters_Table-Order_by_Appearance.tex <==
\begin{table}[!h]
\caption{Summary of notations for sets, parameters, and decision variables.}
\begin{center}
\begin{threeparttable}
\begin{tabular*}{\textwidth}{ l l }
    \toprule
     &  \textbf{Sets} \\
    $I$ & Set of drayage trucks.\\
    $J$ & Set of candidate charging stations.\\
    $K$ & Set of electric substations.\\
    $T$ & Set of time periods in the study time horizon.\\
    $J_{it}$ & Subset of $J$ that truck $i$ has access to at time period $t$.\\
    $J_k$ & Subset of candidate charging stations that can be connected with electric substation $k$.\\
    $K_j$ & Subset of electric substations that can be connected with charging station $j$.\\
    \\
     &  \textbf{Parameters} \\
    $\kappa$ & Cycle efficiency of charging batteries.\\
    $\Delta e^{con}_{it}$ & Energy consumption of truck $i$ at time period $t$.\\
    $r^{stp}_{it}$ & The ratio of time period $t$ that the truck $i$ is parked. \\
    %$SoC^{min/max}$ & Minimal/maximal allowed state-of-charge of an electric truck.\\
    $a_{ijt}$ & $a_{ijt} = 1$ means truck $i$ has access to candidate charging station $j$ during time period $t$. If not, $a_{ijt} = 0$.\\ 
    $p^{max}$ & Maximal charging power for a truck.\\
    $e^{bse}$ & Base battery capacity of an electric truck.\\
    $c^{veh}$ & Cost of one base model electric truck.\\
    $c^{btr}$ & Cost of adding 1kWh of extra battery capacity.\\
    $c^{ele}_t$ & Cost of 1kWh electricity at time $t$.\\
    $c^{ctr}$ & Cost of charging station construction, including planning, permit, civil projects, etc.\\
    $c^{cap}$ & Cost of establishing one kW of power capacity at a charging station.\\
    $c^{chg}$ & Cost of charger per kW basis.\\
    $P^{sbs}_{k}$ & Remaining hosting power capacity of electric substation $k$.\\
    $P^{upg,std}$ & Minimal standard capacity upgrade of a substation.\\
    $PF$ & Typical power factor.\\
    $d_{jk}$ & Distance between charging station $j$ and electric substation $k$.\\
    $c^{lne}$ & Cost of distribution line between a charging station and an electric substation (per mile basis).\\
    $c^{upg,std}$ & Standard fixed cost of substation upgrade.\\
    $c^{upg,var}$ & Variable cost of substation upgrade.\\
    $N_y$ & Targeted number of electric drayage trucks at year $y$.\\
    $u_{i}$ & Daily carbon emission of truck $i$ if it uses diesel as the fuel.\\
    $g_t$ & Electricity carbon intensity of the grid at time $t$.\\
    \\
    & \textbf{Decision Variables$^*$} \\
    $e_{it}$ & (C) Battery energy of truck $i$ at time $t$.\\
    $p_{it}$ & (C) Charging power on truck $i$ at time $t$.\\
    $x_{i}$ & (B) $x_{i} = 1$ indicates truck $i$ is electrified. Otherwise, $x_{i} = 0$.\\
    $e^{cap}_{i}$ & (C) Required battery capacity of truck $i$.\\
    $p^{trk}_{ijt}$ & (C) Charging power supplied by charging station $j$ to truck $i$ at time $t$.\\
    $\hat p^{trk}_{ijt}$ & (B) Binary indicator of whether truck $i$ is charged at station $j$ during time period $t$.\\
    $P_{jt}$ & (C) Power demand of trucks in charging station $j$ at time $t$.\\
    $P^{chs}_{j}$ & (C) Power capacity of charging station $j$.\\
    $\hat P^{chs}_{j}$ & (B) Binary indicator for whether candidate charging station $j$ is deployed.\\
    $P^{chs-sbs}_{jk}$ & (C) Peak power flow between charging station $j$ and electric substation $k$.\\
    $\gamma_{jk}$ & (B) Binary indicator for whether charging station $j$ is connected to electric substation $k$.\\
    $P^{upg}_{k}$ & (C) Total capacity upgrade at substation $k$.\\
    $P^{upg,var}_{k}$ & (C) Variable part of capacity upgrade at substation $k$.\\
    $\hat P^{upg}_{k}$ & (B) Binary indicator for whether there is an upgrade at substation $k$.\\
    \bottomrule
\end{tabular*}
\begin{tablenotes}\footnotesize
\item[*] (C) Continuous variable; (B) Binary variable.
\end{tablenotes}
\end{threeparttable}
\end{center}
\label{tab:params}
\end{table}
